Planetary Nebulae in the Magellanic Clouds: II) Abundances and element production

We present the second part of an optical spectroscopic study of planetary nebulae in the LMC and SMC. The first paper, Leisy & Dennefeld (1996), discussed the CNO cycle for those objects where C abundances were available. In this paper we concentrate more on other elemental abundances (such as O, Ne, S, Ar) and their implications for the evolution of the progenitor stars. We use a much larger sample of 183 objects, of which 65 are from our own observations, where the abundances have been re-derived in a homogeneous way. For 156 of them, the quality of data is considered to be satisfactory for further analysis. We confirm the difficulty of separating Type-I and non-type-I objects in the classical He-N/O diagram, as found in Paper I, a problem reinforced by the variety of initial compositions for the progenitor stars. We observed oxygen variations, either depletion via the ON cycle in the more massive progenitor stars, or oxygen production in other objects. Neon production also appears to be present. These enrichments are best explained by fresh material from the core or from burning shells, brought to the surface by the 3rd dredge-up, as reproduced in recent models, some including overshooting. All the effects appear stronger in the SMC, suggesting a higher efficiency in a low metallicity environment. Neither oxygen nor neon can therefore be used to derive the initial composition of the progenitor star: other elements not affected by processing such as sulfur, argon or, if observed, chlorine, have to be preferred for this purpose. Some objects with very low initial abundances are detected, but on average, the spatial distribution of PNe abundances is consistent with the history of star formation (SF) as derived from field stars in both Clouds.

==> 3063flus.tex <==
 \begin{table}
  \centering
  \label{intensSMC}
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{SMP\_SMC\_1 } & \multicolumn{2}{|c|}{SMP\_SMC\_2 } & \multicolumn{2}{|c|}{SMP\_SMC\_3 } & \multicolumn{2}{|c|}{SMP\_SMC\_4 } & \multicolumn{2}{|c|}{SMP\_SMC\_5 } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  &        -   &        -    &        -   &        -    & $<$   40.0 & $<$  132.1  & $<$   10.0 & $<$  116.2  &        -   &        -   \\
    1550. & CIV             &  2.530  &        -   &        -    &        -   &        -    &      384.0 &     1161.6  & $<$   10.0 & $<$   97.0  &        -   &        -   \\
    1640. & HeII            &  2.319  &        -   &        -    &        -   &        -    & $<$   40.0 & $<$  110.3  & $<$   10.0 & $<$   80.2  &        -   &        -   \\
    1663. & OIII]           &  2.267  &        -   &        -    &        -   &        -    & $<$   40.0 & $<$  107.8  & $<$   10.0 & $<$   76.6  &        -   &        -   \\
    1750. & NIII]           &  2.071  &        -   &        -    &        -   &        -    & $<$   40.0 & $<$   99.0  & $<$   10.0 & $<$   64.2  &        -   &        -   \\
    1909. & CIII]           &  1.793  &        -   &        -    &        -   &        -    &      596.0 &     1305.9  & $<$    5.0 & $<$   25.0  &        -   &        -   \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        -   &        -    &       10.5 &       10.6  &        -   &        -    &        -   &        -    &        9.1 &        9.1 \\
    3427. & [NeV]           &  0.396  &        -   &        -    &       11.2 &       11.3  &        -   &        -    & $<$    5.0 & $<$    7.1  &       17.0 &       17.0 \\
    3727. & [OII]d          &  0.289  &       27.9 &       28.3  &       31.1 &       31.3  &       15.4 &       17.5  &        3.0 &        3.9  &       75.2 &       75.2 \\
    3798. & H10+HeII        &  0.271  &        5.4 &        5.5  &        7.6 &        7.6  &        -   &        -    &        3.0 &        3.8  &        6.1 &        6.1 \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        6.7 &        6.8  &        8.8 &        8.9  &        -   &        -    &        4.2 &        5.3  &        7.2 &        7.2 \\
    3869. & [NeIII]         &  0.253  &        3.9 &        3.9  &       66.9 &       67.3  &       29.5 &       33.0  &       34.4 &       43.2  &       73.2 &       73.2 \\
    3889. & H8+HeI+HeII     &  0.248  &       13.1 &       13.3  &       20.4 &       20.5  &        -   &        -    &       18.0 &       22.5  &       17.4 &       17.4 \\
    3969. & [NeIII]+H7      &  0.229  &       17.8 &       18.0  &       43.6 &       43.8  &        -   &        -    &       22.5 &       27.6  &       40.5 &       40.5 \\
    4026. & HeI+HeII        &  0.216  &        1.7 &        1.7  &        4.8 &        4.8  &        -   &        -    &        2.2 &        2.7  &        -   &        -   \\
    4070. & [SII]d          &  0.207  &        -   &        -    &        -   &        -    &        0.8 &        0.8  &        -   &        -    &        -   &        -   \\
    4102. & Hdelta          &  0.200  &       26.3 &       26.5  &       27.5 &       27.6  &       19.3 &       21.1  &       21.3 &       25.5  &       26.5 &       26.5 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       46.6 &       46.9  &       46.8 &       47.0  &       40.7 &       43.5  &       41.4 &       47.4  &       47.3 &       47.3 \\
    4363. & [OIII]          &  0.147  &        2.1 &        2.1  &       17.4 &       17.5  &        9.3 &        9.9  &       13.0 &       14.8  &       16.1 &       16.1 \\
    4471. & HeI             &  0.112  &        3.1 &        3.1  &        6.3 &        6.3  &        4.8 &        5.0  &        6.0 &        6.7  &        5.7 &        5.7 \\
    4541. & HeII            &  0.091  &        -   &        -    &        3.2 &        3.2  &        -   &        -    &        -   &        -    &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        3.1 &        3.2  &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  & $<$    1.0 & $<$    1.0  &       36.6 &       36.6  & $<$    2.0 & $<$    2.0  & $<$    0.5 & $<$    0.5  &       40.8 &       40.8 \\
    4712. & [ArIV]          &  0.041  & $<$    1.0 & $<$    0.7  &        4.0 &        3.4  & $<$    2.0 & $<$    1.6  &        2.3 &        1.7  &        5.6 &        5.1 \\
    4716. & [NeIV]          &  0.040  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  & $<$    2.0 & $<$    2.0  & $<$    0.5 & $<$    0.5  & $<$    3.0 & $<$    3.0 \\
    4726. & [NeIV]          &  0.037  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  & $<$    2.0 & $<$    2.0  & $<$    0.5 & $<$    0.5  & $<$    3.0 & $<$    3.0 \\
    4741. & [ArIV]          &  0.033  & $<$    1.0 & $<$    1.0  &        3.7 &        3.7  & $<$    2.0 & $<$    2.0  &        1.9 &        2.0  &        3.0 &        3.0 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        -   &        -    &        -   &        -    &        -   &        -    &        0.8 &        0.7  &        -   &        -   \\
    4959. & [OIII]          & -0.025  &       81.5 &       81.4  &      266.0 &      265.8  &      206.0 &      203.7  &      239.0 &      233.6  &      310.0 &      310.0 \\
    5007. & [OIII]          & -0.038  &      236.0 &      235.6  &      763.0 &      762.3  &      607.0 &      597.1  &      713.0 &      689.4  &        -   &        -   \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        2.8 &        2.8  &        -   &        -    &        -   &        -    &        5.5 &        5.5 \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &        -   &        -    &        -   &        -    & $<$    1.0 & $<$    0.9  & $<$    0.3 & $<$    0.3  &        -   &        -   \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       12.7 &       12.6  &       13.2 &       13.1  &       17.0 &       15.4  &       23.3 &       19.1  &       11.5 &       11.5 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        -   &        -    &        1.9 &        1.9  &        -   &        -    &        -   &        -    &        6.8 &        6.8 \\
    6312. & [SIII]+HeII     & -0.296  & $<$    1.0 & $<$    1.0  &        1.5 &        1.5  &        0.7 &        0.6  &        0.6 &        0.4  &        5.0 &        5.0 \\
    6365. & [OI]            & -0.304  &        1.2 &        1.2  &        -   &        -    &        -   &        -    &        -   &        -    &        4.6 &        4.6 \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  &        5.1 &        5.0  &        4.8 &        4.8  &        3.1 &        2.7  &        -   &        -    &       14.5 &       14.5 \\
    6563. & Halpha          & -0.334  &        -   &        -    &      279.0 &      276.9  &      301.0 &      260.1  &      378.0 &      280.1  &      280.0 &      280.0 \\
    6584. & [NII]           & -0.337  &       16.7 &       16.4  &       14.1 &       14.0  &        9.2 &        7.9  &        3.4 &        2.5  &       39.9 &       39.9 \\
    6678. & HeI+HeII        & -0.350  &        2.4 &        2.4  &        3.8 &        3.8  &        4.1 &        3.5  &        6.0 &        4.4  &        4.2 &        4.2 \\
    6716. & [SII]           & -0.356  & $<$    1.0 & $<$    1.0  &        1.7 &        1.7  &        0.4 &        0.4  & $<$    0.3 & $<$    0.2  &        4.5 &        4.5 \\
    6730. & [SII]           & -0.358  & $<$    1.0 & $<$    1.0  &        2.6 &        2.6  &        0.9 &        0.8  & $<$    0.3 & $<$    0.2  &        7.1 &        7.1 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$    1.0 & $<$    1.0  &        0.8 &        0.8  & $<$    1.0 & $<$    0.8  & $<$    0.3 & $<$    0.2  & $<$    3.0 & $<$    3.0 \\
    7065. & HeI             & -0.402  &        7.9 &        7.8  &        6.2 &        6.1  &        -   &        -    &       11.0 &        7.7  &        6.2 &        6.2 \\
    7136. & [ArIII]         & -0.410  &        4.3 &        4.2  &        6.3 &        6.2  &        4.7 &        4.0  &        3.7 &        2.6  &        9.4 &        9.4 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  &       11.7 &       11.5  &        2.8 &        2.8  &        7.0 &        5.8  &        -   &        -    &       10.1 &       10.1 \\
    7330. & [OII]           & -0.434  &        8.3 &        8.1  &        2.4 &        2.4  &        -   &        -    &        -   &        -    &        4.3 &        4.3 \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        2.1 &        2.1  &        -   &        -    &        -   &        -    &        3.8 &        3.8 \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{     871. } & \multicolumn{2}{c}{    1259. } & \multicolumn{2}{c}{ -        } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ 5.0 \%} & \multicolumn{2}{c}{ 3.0 \%} & \multicolumn{2}{c}{ -   \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &  $:$     0.  & &       2954.  & &      21509.  & &  $:$     0.  & &       3218.  & \\
%  &   Ne- [OII]   :    & &      53468.  & &       6336.  & &      18724.  & &          0.  & &       8874.  & \\
%  &   Ne- [ArIV]  :    & &  $:$     0.  & &       5315.  & &  $:$     0.  & &       6045.  & &        100.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{     3000.} & \multicolumn{2}{c}{    21500.} & \multicolumn{2}{c}{     6100.} & \multicolumn{2}{c}{     3200.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    11100.} & \multicolumn{2}{c}{    16200.} & \multicolumn{2}{c}{    13600.} & \multicolumn{2}{c}{    15700.} & \multicolumn{2}{c}{    14500.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{$:$ 11100.} & \multicolumn{2}{c}{$:$ 16200.} & \multicolumn{2}{c}{$:$ 13600.} & \multicolumn{2}{c}{$:$ 15700.} & \multicolumn{2}{c}{$:$ 14500.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.02} & \multicolumn{2}{c}{      0.01} & \multicolumn{2}{c}{      0.19} & \multicolumn{2}{c}{      0.39} & \multicolumn{2}{c}{      0.00} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{SMP\_SMC\_6 } & \multicolumn{2}{|c|}{SMP\_SMC\_7 } & \multicolumn{2}{|c|}{SMP\_SMC\_8 } & \multicolumn{2}{|c|}{SMP\_SMC\_9 } & \multicolumn{2}{|c|}{SMP\_SMC\_10 } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  & $<$   50.0 & $<$ 2799.4  &        -   &        -    &        -   &        -    & $<$  100.0 & $<$  103.1  & $<$   30.0 & $<$  153.9 \\
    1550. & CIV             &  2.530  & $<$   50.0 & $<$ 2080.7  &        -   &        -    &        -   &        -    &      779.0 &      803.0  & $<$   30.0 & $<$  136.4 \\
    1640. & HeII            &  2.319  & $<$   50.0 & $<$ 1523.5  &        -   &        -    &        -   &        -    &      163.0 &      168.0  & $<$   30.0 & $<$  120.2 \\
    1663. & OIII]           &  2.267  & $<$   50.0 & $<$ 1411.2  &        -   &        -    &        -   &        -    & $<$  100.0 & $<$  103.1  & $<$   30.0 & $<$  116.5 \\
    1750. & NIII]           &  2.071  & $<$   50.0 & $<$ 1058.5  &        -   &        -    &        -   &        -    & $<$  100.0 & $<$  103.1  & $<$   30.0 & $<$  103.7 \\
    1909. & CIII]           &  1.793  &      181.0 &     2541.9  &        -   &        -    &        -   &        -    &      915.0 &      943.2  &      263.0 &      769.3 \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  & $<$   10.0 & $<$   17.9  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3727. & [OII]d          &  0.289  &        7.2 &       11.0  &       48.1 &       49.1  &       10.7 &       12.7  &      127.0 &      130.9  &       26.9 &       32.0 \\
    3798. & H10+HeII        &  0.271  &        2.2 &        3.3  &        5.3 &        5.4  &        -   &        -    &        -   &        -    &        4.5 &        5.3 \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        2.9 &        4.2  &        6.4 &        6.5  &        -   &        -    &        -   &        -    &        7.5 &        8.8 \\
    3869. & [NeIII]         &  0.253  &       40.7 &       59.1  &       86.7 &       88.2  &       25.6 &       29.8  &      109.0 &      112.4  &       33.2 &       38.6 \\
    3889. & H8+HeI+HeII     &  0.248  &       11.1 &       16.0  &       23.5 &       23.9  &        -   &        -    &       19.1 &       19.7  &       18.0 &       20.9 \\
    3969. & [NeIII]+H7      &  0.229  &       21.9 &       30.7  &       41.2 &       41.9  &       17.2 &       19.7  &       50.7 &       52.3  &       25.3 &       29.0 \\
    4026. & HeI+HeII        &  0.216  &        1.1 &        1.5  &        -   &        -    &        -   &        -    &        4.6 &        4.8  &        2.6 &        2.9 \\
    4070. & [SII]d          &  0.207  &        1.4 &        2.0  &        2.0 &        2.0  &        -   &        -    &        -   &        -    &        0.6 &        0.7 \\
    4102. & Hdelta          &  0.200  &       17.2 &       23.1  &       25.9 &       26.3  &       13.6 &       15.3  &       33.0 &       33.0  &       25.1 &       28.3 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        1.5 &        1.7 \\
    4340. & Hgamma          &  0.151  &       37.6 &       47.0  &       46.9 &       47.4  &       43.1 &       47.2  &       54.5 &       54.5  &       44.4 &       48.6 \\
    4363. & [OIII]          &  0.147  &       11.3 &       14.0  &       25.2 &       25.5  &        8.1 &        8.8  &       13.6 &       14.0  &        5.3 &        5.8 \\
    4471. & HeI             &  0.112  &        4.6 &        5.5  &        4.3 &        4.3  &        4.1 &        4.4  &        -   &        -    &        3.9 &        4.2 \\
    4541. & HeII            &  0.091  &        -   &        -    &        1.5 &        1.5  &        -   &        -    &        -   &        -    &        -   &        -   \\
    4641. & NIII            &  0.061  &        1.8 &        2.0  &        -   &        -    &        -   &        -    &        -   &        -    &        0.4 &        0.5 \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        1.9 &        2.0  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  & $<$    0.5 & $<$    0.5  &        9.5 &        9.5  &        -   &        -    &       59.6 &       61.4  & $<$    0.1 & $<$    0.1 \\
    4712. & [ArIV]          &  0.041  &        1.1 &        0.6  &        4.4 &        4.0  &        -   &        -    &        3.0 &        3.1  & $<$    0.1 & $<$    0.0 \\
    4716. & [NeIV]          &  0.040  & $<$    0.5 & $<$    0.5  & $<$    1.0 & $<$    1.0  &        -   &        -    & $<$    1.0 & $<$    1.0  & $<$    0.1 & $<$    0.1 \\
    4726. & [NeIV]          &  0.037  & $<$    0.5 & $<$    0.5  &        2.2 &        2.2  &        -   &        -    & $<$    1.0 & $<$    1.0  & $<$    0.1 & $<$    0.1 \\
    4741. & [ArIV]          &  0.033  & $~$    0.9 & $~$    1.0  &        3.8 &        3.8  &        -   &        -    &        3.2 &        3.3  & $<$    0.1 & $<$    0.1 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  & $<$    2.0 & $<$    2.0  &        -   &        -    &        -   &        -    &        -   &        -    &        1.8 &        1.8 \\
    4959. & [OIII]          & -0.025  &      267.0 &      257.2  &      305.0 &      304.5  &      217.0 &      213.7  &      292.0 &      301.0  &      252.0 &      248.2 \\
    5007. & [OIII]          & -0.038  &      829.0 &      784.4  &      934.0 &      931.6  &      630.0 &      616.0  &      874.0 &      900.9  &      609.0 &      595.5 \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        1.4 &        1.4  &        -   &        -    &        3.0 &        3.1  &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &        2.3 &        1.7  &        -   &        -    &        -   &        -    & $<$    1.0 & $<$    1.0  &        0.0 &        0.0 \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       23.8 &       17.1  &        4.6 &        4.5  &       12.8 &       11.2  &        3.5 &        3.6  &       15.5 &       13.6 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        6.2 &        4.0  &        -   &        -    &        -   &        -    &        -   &        -    &        0.4 &        0.4 \\
    6312. & [SIII]+HeII     & -0.296  &        1.5 &        1.0  &        2.1 &        2.1  &        -   &        -    & $<$    1.0 & $<$    1.0  &        0.5 &        0.4 \\
    6365. & [OI]            & -0.304  &        1.4 &        0.9  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  & $<$   25.0 & $<$   15.3  &        4.3 &        4.2  &        -   &        -    & $<$    8.1 & $<$    8.3  &        5.7 &        4.7 \\
    6563. & Halpha          & -0.334  &      456.0 &      278.8  &      274.0 &      267.8  &      282.0 &      230.9  &      231.0 &      231.0  &      359.0 &      294.0 \\
    6584. & [NII]           & -0.337  &       58.8 &       35.8  &       12.9 &       12.6  &        -   &        -    &       17.0 &       17.5  &       12.6 &       10.3 \\
    6678. & HeI+HeII        & -0.350  &        6.9 &        4.1  &        2.8 &        2.7  &        4.6 &        3.7  &        0.7 &        0.7  &        4.5 &        3.7 \\
    6716. & [SII]           & -0.356  &        0.8 &        0.5  &        2.6 &        2.5  &        -   &        -    &        2.8 &        2.9  &        0.7 &        0.6 \\
    6730. & [SII]           & -0.358  &        1.8 &        1.1  &        3.5 &        3.4  &        -   &        -    &        4.1 &        4.2  &        1.0 &        0.8 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$    0.5 & $<$    0.3  & $<$    1.0 & $<$    1.0  &        -   &        -    & $<$    1.0 & $<$    1.0  &        -   &        -   \\
    7065. & HeI             & -0.402  &       21.4 &       11.8  &        4.0 &        3.9  &        6.2 &        4.9  &        -   &        -    &        6.2 &        4.8 \\
    7136. & [ArIII]         & -0.410  &       14.4 &        7.9  &        2.4 &        2.3  &        2.3 &        1.8  &        4.2 &        4.4  &        5.7 &        4.4 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        2.0 &        1.1  &        -   &        -    &        -   &        -    &        -   &        -    &        1.2 &        0.9 \\
    7320. & [OII]           & -0.433  &       12.2 &        6.4  &        -   &        -    &        -   &        -    & $<$    1.0 & $<$    1.0  &        1.3 &        1.0 \\
    7330. & [OII]           & -0.434  &        6.6 &        3.5  &        -   &        -    &        -   &        -    & $<$    1.0 & $<$    1.0  &        1.2 &        0.9 \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        1.1 &        0.8 \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        6.8 &        4.8 \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &       12.1 &        8.3 \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{    1585. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{     372. } & \multicolumn{2}{c}{    1175. } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ 2.0 \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ 5.0 \%} & \multicolumn{2}{c}{ 1.0 \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &      99690.  & &       1947.  & &          0.  & &       2217.  & &       1914.  & \\
%  &   Ne- [OII]   :    & &      48752.  & &  $<$*******  & &      10970.  & &  $<$*******  & &       2453.  & \\
%  &   Ne- [ArIV]  :    & &      11345.  & &       3539.  & &          0.  & &       4551.  & &  $:$     0.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{    11400.} & \multicolumn{2}{c}{     1900.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{     2200.} & \multicolumn{2}{c}{     1500.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    14400.} & \multicolumn{2}{c}{    17900.} & \multicolumn{2}{c}{    13200.} & \multicolumn{2}{c}{    13700.} & \multicolumn{2}{c}{    11300.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{    15600.} & \multicolumn{2}{c}{$:$ 17900.} & \multicolumn{2}{c}{$:$ 13200.} & \multicolumn{2}{c}{$~$ 13700.} & \multicolumn{2}{c}{    11300.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.64} & \multicolumn{2}{c}{      0.03} & \multicolumn{2}{c}{      0.26} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.26} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{SMP\_SMC\_11 } & \multicolumn{2}{|c|}{SMP\_SMC\_12 } & \multicolumn{2}{|c|}{SMP\_SMC\_13 } & \multicolumn{2}{|c|}{SMP\_SMC\_14 } & \multicolumn{2}{|c|}{SMP\_SMC\_15 } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  &        -   &        -    &        -   &        -    & $<$   30.0 & $<$   82.1  & $<$   50.0 & $<$  309.8  &        -   &        -   \\
    1550. & CIV             &  2.530  &        -   &        -    &        -   &        -    & $<$   40.0 & $<$  101.6  &      864.0 &     4679.8  &        -   &        -   \\
    1640. & HeII            &  2.319  &        -   &        -    &        -   &        -    & $<$   20.0 & $<$   47.0  &      130.0 &      611.4  &        -   &        -   \\
    1663. & OIII]           &  2.267  &        -   &        -    &        -   &        -    & $<$   20.0 & $<$   46.1  & $<$   40.0 & $<$  181.7  &        -   &        -   \\
    1750. & NIII]           &  2.071  &        -   &        -    &        -   &        -    & $<$   20.0 & $<$   42.9  & $<$   40.0 & $<$  159.5  &        -   &        -   \\
    1909. & CIII]           &  1.793  &        -   &        -    &        -   &        -    &      390.0 &      755.0  &      730.0 &     2417.0  &        -   &        -   \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  & $<$   10.0 & $<$   21.1  & $<$   10.0 & $<$   13.8  &        -   &        -    &        -   &        -    &        -   &        -   \\
    3727. & [OII]d          &  0.289  &       94.4 &      162.8  & $<$    3.0 & $<$    3.8  &       12.5 &       13.9  &       29.6 &       35.9  &       13.7 &       14.1 \\
    3798. & H10+HeII        &  0.271  &        -   &        -    &        -   &        -    &        -   &        -    &        3.7 &        4.4  &        4.9 &        5.0 \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        1.6 &        1.6 \\
    3835. & H9+HeII         &  0.261  &        -   &        -    &        -   &        -    &        4.3 &        4.7  &        6.0 &        7.1  &        7.5 &        7.7 \\
    3869. & [NeIII]         &  0.253  & $<$   10.0 & $<$   16.1  &       20.9 &       25.6  &       29.7 &       32.6  &       46.9 &       55.5  &       48.1 &       49.2 \\
    3889. & H8+HeI+HeII     &  0.248  &        -   &        -    &       18.2 &       22.2  &       10.1 &       11.1  &       10.4 &       12.3  &       16.7 &       17.1 \\
    3969. & [NeIII]+H7      &  0.229  &        -   &        -    &       17.1 &       20.6  &       20.5 &       22.3  &       21.7 &       25.3  &       26.4 &       27.0 \\
    4026. & HeI+HeII        &  0.216  &        -   &        -    &        -   &        -    &        1.9 &        2.1  &        -   &        -    &        3.1 &        3.2 \\
    4070. & [SII]d          &  0.207  &        -   &        -    &        -   &        -    &        0.8 &        0.9  &        -   &        -    &        1.0 &        1.0 \\
    4102. & Hdelta          &  0.200  &       13.6 &       19.8  &       19.5 &       22.9  &       19.2 &       20.7  &       20.1 &       23.0  &       27.3 &       27.8 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        0.8 &        0.8  &        -   &        -    &        0.5 &        0.5 \\
    4340. & Hgamma          &  0.151  &       33.7 &       44.8  &       41.3 &       46.6  &       42.7 &       45.1  &       42.7 &       47.2  &       46.5 &       47.2 \\
    4363. & [OIII]          &  0.147  & $<$    2.0 & $<$    2.6  &        7.4 &        8.3  &        9.4 &        9.9  &       12.5 &       13.8  &        6.4 &        6.5 \\
    4471. & HeI             &  0.112  &        -   &        -    &        6.1 &        6.6  &        4.3 &        4.5  &        2.5 &        2.7  &        5.8 &        5.9 \\
    4541. & HeII            &  0.091  &        -   &        -    &        -   &        -    &        -   &        -    &        1.4 &        1.4  &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    & $~$    1.5 & $~$    1.6  &        -   &        -   \\
    4659. & CIV             &  0.056  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  & $<$    1.0 & $<$    1.1  & $<$    2.0 & $<$    2.1  & $<$    0.3 & $<$    0.3  &       37.8 &       39.0  & $<$    1.0 & $<$    1.0 \\
    4712. & [ArIV]          &  0.041  & $<$    1.0 & $<$    1.1  & $<$    2.0 & $<$    1.5  &        1.2 &        0.8  &        2.5 &        2.3  &        1.2 &        0.7 \\
    4716. & [NeIV]          &  0.040  & $<$    1.0 & $<$    1.1  & $<$    2.0 & $<$    2.1  & $<$    0.3 & $<$    0.3  & $<$    0.5 & $<$    0.5  & $<$    1.0 & $<$    1.0 \\
    4726. & [NeIV]          &  0.037  & $<$    1.0 & $<$    1.1  & $<$    2.0 & $<$    2.1  & $<$    0.3 & $<$    0.3  & $<$    0.5 & $<$    0.5  & $<$    1.0 & $<$    1.0 \\
    4741. & [ArIV]          &  0.033  & $<$    1.0 & $<$    1.1  & $<$    2.0 & $<$    2.1  &        0.6 &        0.6  &        2.1 &        2.2  & $<$    1.0 & $<$    1.0 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        1.4 &        1.4 \\
    4959. & [OIII]          & -0.025  &      123.0 &      117.2  &      199.0 &      195.0  &      268.0 &      265.5  &      307.0 &      301.8  &      201.0 &      200.5 \\
    5007. & [OIII]          & -0.038  &      375.0 &      349.3  &      599.0 &      581.1  &      805.0 &      793.9  &      905.0 &      882.6  &        -   &        -   \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        -   &        -    &        -   &        -    &        2.4 &        2.2  &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  & $<$    1.0 & $<$    0.7  & $<$    1.0 & $<$    0.9  & $<$    0.4 & $<$    0.4  & $<$    0.4 & $<$    0.3  &        0.5 &        0.5 \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       17.0 &       11.2  &       16.6 &       13.9  &       17.0 &       15.7  &        9.4 &        8.1  &       15.1 &       14.8 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        1.9 &        1.1  &        -   &        -    &        2.7 &        2.4  &        3.4 &        2.8  &        2.2 &        2.1 \\
    6312. & [SIII]+HeII     & -0.296  &        3.0 &        1.7  & $<$    1.0 & $<$    0.8  &        0.6 &        0.6  &        1.0 &        0.8  &        0.9 &        0.9 \\
    6365. & [OI]            & -0.304  &        -   &        -    &        -   &        -    &        1.0 &        0.9  &        -   &        -    &        0.9 &        0.9 \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  &       11.7 &        6.3  &        -   &        -    & $<$    6.5 & $<$    5.8  & $<$    6.1 & $<$    4.9  &        3.8 &        3.7 \\
    6563. & Halpha          & -0.334  &      509.0 &      271.0  &      364.0 &      278.1  &      307.0 &      271.5  &      278.0 &      222.4  &      284.0 &      275.4 \\
    6584. & [NII]           & -0.337  &       27.7 &       14.7  &        1.8 &        1.4  &       13.4 &       11.8  &       11.9 &        9.5  &       11.5 &       11.1 \\
    6678. & HeI+HeII        & -0.350  &        7.7 &        4.0  &        4.9 &        3.7  &        4.2 &        3.7  &        2.3 &        1.8  &        3.5 &        3.4 \\
    6716. & [SII]           & -0.356  &        6.5 &        3.3  & $<$    1.0 & $<$    0.8  &        0.6 &        0.5  &        1.0 &        0.8  & $<$    1.0 & $<$    1.0 \\
    6730. & [SII]           & -0.358  &        7.0 &        3.6  & $<$    1.0 & $<$    0.7  &        1.1 &        1.0  &        1.4 &        1.1  & $<$    1.0 & $<$    1.0 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$    2.0 & $<$    0.9  & $<$    1.0 & $<$    0.7  & $<$    0.3 & $<$    0.3  & $<$    0.5 & $<$    0.4  & $<$    1.0 & $<$    1.0 \\
    7065. & HeI             & -0.402  &       15.7 &        7.4  &        5.8 &        4.2  &       11.8 &       10.2  &        2.9 &        2.2  &        7.8 &        7.5 \\
    7136. & [ArIII]         & -0.410  &       17.3 &        8.0  &        2.2 &        1.6  &        4.6 &        4.0  &        3.7 &        2.8  &        4.9 &        4.7 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        -   &        -    &        -   &        -    &        1.0 &        0.8  &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  &        -   &        -    & $<$    1.0 & $<$    0.7  &        3.3 &        2.8  &        -   &        -    &        -   &        -   \\
    7330. & [OII]           & -0.434  &        -   &        -    & $<$    1.0 & $<$    0.7  &        3.4 &        2.9  &        -   &        -    &        -   &        -   \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{    1349. } & \multicolumn{2}{c}{     355. } & \multicolumn{2}{c}{    2754. } & \multicolumn{2}{c}{    1000. } & \multicolumn{2}{c}{ -        } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ 8.0 \%} & \multicolumn{2}{c}{11.0 \%} & \multicolumn{2}{c}{ 1.0 \%} & \multicolumn{2}{c}{ 2.0 \%} & \multicolumn{2}{c}{ -   \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &        791.  & &  $:$     0.  & &      10720.  & &       1872.  & &  $:$     0.  & \\
%  &   Ne- [OII]   :    & &       6041.  & &  $:$     0.  & &      26549.  & &         70.  & &  $<$  1373.  & \\
%  &   Ne- [ArIV]  :    & &  $:$     0.  & &  $:$     0.  & &        100.  & &       3222.  & &  $<$  9998.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{      800.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{    10700.} & \multicolumn{2}{c}{     1900.} & \multicolumn{2}{c}{$*$  5000.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{    13200.} & \multicolumn{2}{c}{    12400.} & \multicolumn{2}{c}{    13700.} & \multicolumn{2}{c}{    12000.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$:$ 13200.} & \multicolumn{2}{c}{$~$ 12400.} & \multicolumn{2}{c}{$~$ 13700.} & \multicolumn{2}{c}{    16200.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.82} & \multicolumn{2}{c}{      0.35} & \multicolumn{2}{c}{      0.16} & \multicolumn{2}{c}{      0.29} & \multicolumn{2}{c}{      0.04} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{SMP\_SMC\_16 } & \multicolumn{2}{|c|}{SMP\_SMC\_17 } & \multicolumn{2}{|c|}{SMP\_SMC\_18 } & \multicolumn{2}{|c|}{SMP\_SMC\_19 } & \multicolumn{2}{|c|}{SMP\_SMC\_20 } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  &        -   &        -    &        -   &        -    &        -   &        -    & $<$   30.0 & $<$  112.4  & $<$   15.0 & $<$   20.5 \\
    1550. & CIV             &  2.530  &        -   &        -    &        -   &        -    &        -   &        -    &      209.0 &      710.3  & $<$   15.0 & $<$   20.1 \\
    1640. & HeII            &  2.319  &        -   &        -    &        -   &        -    &        -   &        -    &       67.0 &      205.6  & $<$   15.0 & $<$   19.6 \\
    1663. & OIII]           &  2.267  &        -   &        -    &        -   &        -    &        -   &        -    & $<$   30.0 & $<$   89.8  & $<$   15.0 & $<$   19.5 \\
    1750. & NIII]           &  2.071  &        -   &        -    &        -   &        -    &        -   &        -    & $<$   30.0 & $<$   81.7  & $<$   15.0 & $<$   19.0 \\
    1909. & CIII]           &  1.793  &        -   &        -    &        -   &        -    &        -   &        -    &      357.0 &      849.5  &      431.0 &      529.8 \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3727. & [OII]d          &  0.289  &      101.0 &      101.0  &       33.6 &       33.6  &       85.7 &       85.7  &       16.5 &       19.0  &        2.5 &        2.6 \\
    3798. & H10+HeII        &  0.271  &        5.9 &        5.9  &        5.0 &        5.0  &        -   &        -    &        -   &        -    &        3.5 &        3.6 \\
    3820. & HeI             &  0.265  &        1.6 &        1.6  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        5.9 &        5.9  &        8.1 &        8.1  &        -   &        -    &        -   &        -    &        6.9 &        7.1 \\
    3869. & [NeIII]         &  0.253  &        2.7 &        2.7  &       79.6 &       79.6  &       24.6 &       24.6  &       41.2 &       46.6  &       16.6 &       17.1 \\
    3889. & H8+HeI+HeII     &  0.248  &       17.5 &       17.5  &       24.8 &       24.8  &        -   &        -    &       12.1 &       13.6  &       13.3 &       13.7 \\
    3969. & [NeIII]+H7      &  0.229  &       18.3 &       18.3  &       46.5 &       46.5  &       25.3 &       25.3  &       20.9 &       23.4  &       18.8 &       19.3 \\
    4026. & HeI+HeII        &  0.216  &        2.4 &        2.4  &        2.3 &        2.3  &        -   &        -    &        -   &        -    &        1.7 &        1.8 \\
    4070. & [SII]d          &  0.207  &        1.5 &        1.5  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4102. & Hdelta          &  0.200  &       25.0 &       25.0  &       36.5 &       36.5  &       27.6 &       27.6  &       21.3 &       23.5  &       23.4 &       23.9 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       47.3 &       47.3  &       60.1 &       60.1  &       49.5 &       49.5  &       42.0 &       45.2  &       46.4 &       47.2 \\
    4363. & [OIII]          &  0.147  &        1.8 &        1.8  &       15.1 &       15.1  &        2.4 &        2.4  & $<$    0.5 & $<$    0.5  &        5.6 &        5.7 \\
    4471. & HeI             &  0.112  &        3.2 &        3.2  &        7.8 &        7.8  &        4.6 &        4.6  &        2.2 &        2.4  &        4.8 &        4.9 \\
    4541. & HeII            &  0.091  &        -   &        -    &        -   &        -    &        -   &        -    &        0.9 &        1.0  &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        1.3 &        1.3  &        -   &        -   \\
    4659. & CIV             &  0.056  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  &        -   &        -    &       40.0 &       40.9  & $<$    0.3 & $<$    0.3 \\
    4712. & [ArIV]          &  0.041  &        1.1 &        0.8  & $<$    1.0 & $<$    0.3  &        -   &        -    &        2.6 &        2.5  &        0.7 &        0.2 \\
    4716. & [NeIV]          &  0.040  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  &        -   &        -    & $<$    2.0 & $<$    2.0  & $<$    0.3 & $<$    0.3 \\
    4726. & [NeIV]          &  0.037  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  &        -   &        -    & $<$    2.0 & $<$    2.0  & $<$    0.3 & $<$    0.3 \\
    4741. & [ArIV]          &  0.033  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  &        -   &        -    &        2.2 &        2.2  & $<$    0.3 & $<$    0.3 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        0.9 &        0.9 \\
    4959. & [OIII]          & -0.025  &       60.8 &       60.8  &      277.0 &      277.0  &      107.0 &      107.0  &      276.0 &      272.6  &      139.0 &      138.6 \\
    5007. & [OIII]          & -0.038  &      167.0 &      167.0  &        -   &        -    &      294.0 &      294.0  &      838.0 &      822.9  &      422.0 &      420.2 \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        -   &        -    &        -   &        -    &        3.0 &        2.8  &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &        -   &        -    &        -   &        -    &        -   &        -    & $<$    0.5 & $<$    0.5  & $<$    0.4 & $<$    0.4 \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &        8.3 &        8.3  &       15.7 &       15.7  &       12.6 &       12.6  &        9.3 &        8.4  &       16.0 &       15.6 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        0.5 &        0.5  &        -   &        -    &        3.4 &        3.4  &        1.7 &        1.5  &        0.9 &        0.9 \\
    6312. & [SIII]+HeII     & -0.296  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  &        -   &        -    & $<$    1.0 & $<$    0.9  & $<$    0.4 & $<$    0.4 \\
    6365. & [OI]            & -0.304  &        0.4 &        0.4  &        -   &        -    &        -   &        -    &        -   &        -    &        0.4 &        0.4 \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  &        4.5 &        4.5  &        -   &        -    &        4.8 &        4.8  & $<$    8.0 & $<$    6.8  &        1.5 &        1.4 \\
    6563. & Halpha          & -0.334  &        -   &        -    &        -   &        -    &      283.0 &      283.0  &      321.0 &      273.1  &      269.0 &      258.9 \\
    6584. & [NII]           & -0.337  &       13.0 &       13.0  &       35.1 &       35.1  &       14.0 &       14.0  &       13.8 &       11.7  &        4.0 &        3.9 \\
    6678. & HeI+HeII        & -0.350  &        1.2 &        1.2  &        5.2 &        5.2  &        2.8 &        2.8  &        2.9 &        2.4  &        3.3 &        3.2 \\
    6716. & [SII]           & -0.356  & $<$    1.0 & $<$    1.0  &        0.4 &        0.4  &        -   &        -    &        0.5 &        0.4  & $<$    0.5 & $<$    0.5 \\
    6730. & [SII]           & -0.358  & $<$    1.0 & $<$    1.0  &        1.7 &        1.7  &        -   &        -    &        1.2 &        1.0  & $<$    0.5 & $<$    0.5 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$    1.0 & $<$    1.0  & $<$    1.0 & $<$    1.0  &        -   &        -    & $<$    1.0 & $<$    0.8  & $<$    0.5 & $<$    0.5 \\
    7065. & HeI             & -0.402  &        3.3 &        3.3  &       11.4 &       11.4  &        8.7 &        8.7  &        3.1 &        2.6  &        9.7 &        9.2 \\
    7136. & [ArIII]         & -0.410  &        1.5 &        1.5  &        6.7 &        6.7  &        6.8 &        6.8  &        2.9 &        2.4  &        1.9 &        1.8 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        0.5 &        0.5  &        -   &        -    &        -   &        -    &        -   &        -    &        1.3 &        1.2 \\
    7320. & [OII]           & -0.433  &        5.1 &        5.1  &        4.4 &        4.4  &        -   &        -    &        2.5 &        2.0  &        3.3 &        3.1 \\
    7330. & [OII]           & -0.434  &        2.7 &        2.7  &        1.6 &        1.6  &        -   &        -    &        2.4 &        1.9  &        3.0 &        2.8 \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{    1175. } & \multicolumn{2}{c}{    3802. } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ 3.0 \%} & \multicolumn{2}{c}{ 1.0 \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &  $:$     0.  & &     300000.  & &          0.  & &     300000.  & &  $:$     0.  & \\
%  &   Ne- [OII]   :    & &       3385.  & &       7899.  & &      15624.  & &      12744.  & &     156211.  & \\
%  &   Ne- [ArIV]  :    & &  $<$  6578.  & &  $:$     0.  & &          0.  & &       2324.  & &  $<$  7885.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{     2300.} & \multicolumn{2}{c}{$*$  5000.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    11800.} & \multicolumn{2}{c}{    14800.} & \multicolumn{2}{c}{    10700.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{    12900.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{$:$ 11800.} & \multicolumn{2}{c}{$:$ 14800.} & \multicolumn{2}{c}{$:$ 10700.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$:$ 12900.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.21} & \multicolumn{2}{c}{      0.05} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{SMP\_SMC\_21 } & \multicolumn{2}{|c|}{SMP\_SMC\_22 } & \multicolumn{2}{|c|}{SMP\_SMC\_23 } & \multicolumn{2}{|c|}{SMP\_SMC\_24 } & \multicolumn{2}{|c|}{SMP\_SMC\_25 } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  & $<$  100.0 & $<$ 1162.1  &       10.4 &      160.3  & $<$   30.0 & $<$   52.8  &        -   &        -    & $<$   20.0 & $<$   87.3 \\
    1550. & CIV             &  2.530  & $<$  100.0 & $<$  969.9  &       90.0 &     1136.4  &      167.0 &      282.1  &        -   &        -    & $<$   20.0 & $<$   78.5 \\
    1640. & HeII            &  2.319  & $~$  152.0 & $~$ 1219.2  &      208.0 &     2130.1  & $<$   30.0 & $<$   48.5  &        -   &        -    & $~$   27.2 & $~$   95.4 \\
    1663. & OIII]           &  2.267  & $<$  100.0 & $<$  765.6  &       62.3 &      606.0  & $<$   30.0 & $<$   48.0  &        -   &        -    & $<$   20.0 & $<$   68.3 \\
    1750. & NIII]           &  2.071  & $<$  100.0 & $<$  642.5  &       93.4 &      748.9  & $<$   30.0 & $<$   46.1  &        -   &        -    & $<$   20.0 & $<$   61.6 \\
    1909. & CIII]           &  1.793  & $<$   50.0 & $<$  250.2  &       38.1 &      231.9  &      295.0 &      427.7  &        -   &        -    & $<$   20.0 & $<$   53.1 \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &       16.7 &       22.3 \\
    3347. & [NeV]           &  0.431  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &       34.9 &       45.1 \\
    3427. & [NeV]           &  0.396  & $<$   50.0 & $<$   71.4  &        -   &        -    &        -   &        -    &        -   &        -    &      102.0 &      129.3 \\
    3727. & [OII]d          &  0.289  &       14.2 &       18.4  &       31.7 &       43.5  & $<$   10.0 & $<$   10.6  &       85.6 &       85.6  &        8.9 &       10.6 \\
    3798. & H10+HeII        &  0.271  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        2.3 &        2.7 \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        -   &        -    &        3.1 &        4.2  &        -   &        -    &        -   &        -    &        5.6 &        6.6 \\
    3869. & [NeIII]         &  0.253  &       47.5 &       59.6  &       20.4 &       27.0  &       53.5 &       56.4  &       26.1 &       26.1  &       41.4 &       48.6 \\
    3889. & H8+HeI+HeII     &  0.248  &       20.9 &       26.1  &       10.6 &       14.0  &       18.1 &       19.1  &        -   &        -    &       18.9 &       22.1 \\
    3969. & [NeIII]+H7      &  0.229  &       35.2 &       43.2  &       15.6 &       20.2  &       30.7 &       32.2  &       24.5 &       24.5  &       26.9 &       31.2 \\
    4026. & HeI+HeII        &  0.216  &        -   &        -    &        1.2 &        1.6  &        1.2 &        1.3  &        -   &        -    &        -   &        -   \\
    4070. & [SII]d          &  0.207  &        7.7 &        9.3  &        2.4 &        3.0  &        -   &        -    &        -   &        -    &        2.9 &        3.3 \\
    4102. & Hdelta          &  0.200  &       23.6 &       28.2  &       17.2 &       21.0  &       25.3 &       26.4  &       24.2 &       24.2  &       23.0 &       25.6 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       43.5 &       49.8  &       37.3 &       43.3  &       45.8 &       47.3  &       50.8 &       50.8  &       45.2 &       49.0 \\
    4363. & [OIII]          &  0.147  &       20.9 &       23.8  &       11.5 &       13.7  &       10.2 &       10.5  &        6.0 &        6.0  &       18.9 &       21.0 \\
    4471. & HeI             &  0.112  &        5.1 &        5.6  &        3.8 &        4.4  &        4.8 &        5.0  &        8.2 &        8.2  &        3.1 &        3.4 \\
    4541. & HeII            &  0.091  &        -   &        -    &        1.9 &        2.1  &        -   &        -    &        -   &        -    &        1.8 &        2.0 \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        6.0 &        6.3  &        1.1 &        1.2  &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  &       38.4 &       40.1  &       60.4 &       65.3  &        2.8 &        2.8  &        -   &        -    &       53.3 &       56.2 \\
    4712. & [ArIV]          &  0.041  &        4.2 &        3.9  &        4.9 &        4.8  &        1.7 &        1.3  &        -   &        -    & $~$    3.5 & $~$    3.4 \\
    4716. & [NeIV]          &  0.040  & $<$    4.0 & $<$    4.1  & $<$    1.0 & $<$    1.1  & $<$    1.0 & $<$    1.0  &        -   &        -    & $~$    1.2 & $~$    1.3 \\
    4726. & [NeIV]          &  0.037  & $<$    4.0 & $<$    4.1  & $<$    1.0 & $<$    1.1  & $<$    1.0 & $<$    1.0  &        -   &        -    & $~$    1.2 & $~$    1.3 \\
    4741. & [ArIV]          &  0.033  &        7.5 &        7.7  &        3.4 &        3.6  & $<$    1.0 & $<$    1.0  &        -   &        -    &        4.3 &        4.5 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4959. & [OIII]          & -0.025  &      173.0 &      169.1  &       96.9 &       97.4  &      265.0 &      263.6  &      155.0 &      155.0  &      107.0 &      108.5 \\
    5007. & [OIII]          & -0.038  &      540.0 &      522.1  &      306.0 &      304.0  &      798.0 &      791.8  &      457.0 &      457.0  &      314.0 &      316.3 \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &       13.8 &       13.1  &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        5.8 &        5.2  &        -   &        -    &        -   &        -    &        2.9 &        2.8 \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  & $~$    5.8 & $~$    4.8  &        6.1 &        5.2  & $<$    0.5 & $<$    0.5  &        -   &        -    &        3.6 &        3.3 \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       22.1 &       18.1  &       14.9 &       12.3  &       15.1 &       14.4  &       12.4 &       12.4  &       12.6 &       11.5 \\
    6088. & [CaV]+[FeVII]   & -0.260  &       11.8 &        9.3  &        2.2 &        1.8  &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        3.3 &        2.5  &       14.3 &       11.0  &        -   &        -    &        1.6 &        1.6  &        2.9 &        2.5 \\
    6312. & [SIII]+HeII     & -0.296  &        3.8 &        2.9  & $~$    2.8 & $~$    2.2  & $<$    0.5 & $<$    0.5  &        -   &        -    &        1.7 &        1.5 \\
    6365. & [OI]            & -0.304  &        -   &        -    &        4.2 &        3.2  &        -   &        -    &        -   &        -    &        -   &        -   \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        0.8 &        0.6  &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  & $<$   64.0 & $<$   47.5  & $<$   99.8 & $<$   74.1  &        -   &        -    &        5.0 &        5.0  & $~$   23.0 & $~$   19.8 \\
    6563. & Halpha          & -0.334  &      383.0 &      283.8  &      345.0 &      247.9  &      305.0 &      284.6  &      282.0 &      282.0  &      338.0 &      283.2 \\
    6584. & [NII]           & -0.337  &      142.0 &      104.9  &      275.0 &      203.1  &        3.7 &        3.5  &       14.7 &       14.7  &       54.7 &       47.0 \\
    6678. & HeI+HeII        & -0.350  &        -   &        -    &        4.0 &        2.9  &        3.5 &        3.3  &        2.6 &        2.6  &        3.6 &        3.0 \\
    6716. & [SII]           & -0.356  &        6.6 &        4.8  &       10.2 &        7.4  & $<$    0.5 & $<$    0.5  &        1.8 &        1.8  & $<$    2.0 & $<$    1.7 \\
    6730. & [SII]           & -0.358  &       13.2 &        9.6  &       13.6 &        9.8  & $<$    0.5 & $<$    0.5  &        -   &        -    & $<$    2.0 & $<$    1.7 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$    5.0 & $<$    3.5  &        1.7 &        1.2  & $<$    0.5 & $<$    0.5  &        -   &        -    & $<$    2.0 & $<$    1.7 \\
    7065. & HeI             & -0.402  &       20.5 &       14.3  &        6.8 &        4.7  &        5.6 &        5.1  &        -   &        -    &        6.5 &        5.4 \\
    7136. & [ArIII]         & -0.410  &        9.6 &        6.7  &        6.0 &        4.1  &        3.1 &        2.8  &        -   &        -    &        4.3 &        3.6 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        -   &        -    &        1.0 &        0.7  &        -   &        -    &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  & $<$    5.0 & $<$    3.4  &        1.4 &        0.9  &        -   &        -    &        -   &        -    & $<$    3.5 & $<$    2.9 \\
    7330. & [OII]           & -0.434  & $<$    5.0 & $<$    3.4  &        5.0 &        3.3  &        -   &        -    &        -   &        -    & $<$    3.5 & $<$    2.9 \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{     562. } & \multicolumn{2}{c}{    1318. } & \multicolumn{2}{c}{     871. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{     631. } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{10.0 \%} & \multicolumn{2}{c}{ 2.0 \%} & \multicolumn{2}{c}{ 3.0 \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ 6.0 \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &      10226.  & &       1678.  & &  $:$     0.  & &          0.  & &  $:$     0.  & \\
%  &   Ne- [OII]   :    & &  $<$ 18072.  & &       4601.  & &  $:$     0.  & &          0.  & &  $<$ 22505.  & \\
%  &   Ne- [ArIV]  :    & &      22359.  & &        552.  & &  $<$   939.  & &          0.  & &       9702.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{    10200.} & \multicolumn{2}{c}{     1700.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{     9800.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    24400.} & \multicolumn{2}{c}{    24700.} & \multicolumn{2}{c}{    12800.} & \multicolumn{2}{c}{    12700.} & \multicolumn{2}{c}{$:$ 21100.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{    15700.} & \multicolumn{2}{c}{    12200.} & \multicolumn{2}{c}{$:$ 12800.} & \multicolumn{2}{c}{$:$ 12700.} & \multicolumn{2}{c}{    21100.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.39} & \multicolumn{2}{c}{      0.43} & \multicolumn{2}{c}{      0.09} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.23} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{SMP\_SMC\_26 } & \multicolumn{2}{|c|}{SMP\_SMC\_27 } & \multicolumn{2}{|c|}{SMP\_SMC\_28 } & \multicolumn{2}{|c|}{SMP\_SMC\_32 } & \multicolumn{2}{|c|}{SMP\_SMC\_34 } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  &        -   &        -    &        -   &        -    &      150.0 &      508.8  &        -   &        -    &        -   &        -   \\
    1550. & CIV             &  2.530  &        -   &        -    &        -   &        -    & $<$   10.0 & $<$   31.1  &        -   &        -    &        -   &        -   \\
    1640. & HeII            &  2.319  &        -   &        -    &        -   &        -    &      152.0 &      430.4  &        -   &        -    &        -   &        -   \\
    1663. & OIII]           &  2.267  &        -   &        -    &        -   &        -    &       30.0 &       83.0  &        -   &        -    &        -   &        -   \\
    1750. & NIII]           &  2.071  &        -   &        -    &        -   &        -    &      191.0 &      485.4  &        -   &        -    &        -   &        -   \\
    1909. & CIII]           &  1.793  &        -   &        -    &        -   &        -    & $<$   10.0 & $<$   22.5  &        -   &        -    &        -   &        -   \\
    3203. & HeII            &  0.498  &       16.2 &       27.6  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        7.5 &       11.9  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  &       22.9 &       35.1  &        -   &        -    &        -   &        -    & $<$   10.0 & $<$   10.0  & $<$   10.0 & $<$   10.3 \\
    3727. & [OII]d          &  0.289  &      117.0 &      161.0  &       16.9 &       16.9  & $<$   10.0 & $<$   11.7  & $<$    4.0 & $<$    4.0  &      232.0 &      236.7 \\
    3798. & H10+HeII        &  0.271  &        -   &        -    &        -   &        -    &        -   &        -    &        4.6 &        4.6  &        -   &        -   \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        4.6 &        6.2  &        -   &        -    &        -   &        -    &        8.0 &        8.0  &        -   &        -   \\
    3869. & [NeIII]         &  0.253  &       48.3 &       64.1  &       31.2 &       31.2  &       35.2 &       40.4  &       40.7 &       40.7  &       48.2 &       49.0 \\
    3889. & H8+HeI+HeII     &  0.248  &       19.8 &       26.1  &       15.6 &       15.6  &       16.5 &       18.9  &       19.6 &       19.6  &       22.4 &       22.8 \\
    3969. & [NeIII]+H7      &  0.229  &       27.1 &       35.1  &       20.9 &       20.9  &       25.4 &       28.8  &       30.0 &       30.0  &       31.0 &       31.5 \\
    4026. & HeI+HeII        &  0.216  &        -   &        -    &        -   &        -    &        -   &        -    &        3.3 &        3.3  &        1.2 &        1.2 \\
    4070. & [SII]d          &  0.207  &        4.3 &        5.4  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4102. & Hdelta          &  0.200  &       22.0 &       26.9  &       25.6 &       25.6  &       19.2 &       21.0  &       28.1 &       28.1  &       29.7 &       30.1 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       41.6 &       48.5  &       47.4 &       47.4  &       44.0 &       47.0  &       52.6 &       52.6  &       46.6 &       47.1 \\
    4363. & [OIII]          &  0.147  &       13.3 &       15.8  &        8.7 &        8.7  &        8.4 &        9.2  &       12.9 &       12.9  &        5.8 &        5.9 \\
    4471. & HeI             &  0.112  &        2.3 &        2.7  &        3.1 &        3.1  & $~$    5.6 & $~$    6.0  &        3.6 &        3.6  &        3.0 &        3.0 \\
    4541. & HeII            &  0.091  &        1.3 &        1.4  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  &       52.5 &       56.6  &        -   &        -    &       52.1 &       54.6  &       12.1 &       12.1  &       10.3 &       10.3 \\
    4712. & [ArIV]          &  0.041  &        2.5 &        2.3  &        2.7 &        2.4  &        3.7 &        3.3  & $<$    2.0 & $<$    1.7  & $<$    1.0 & $<$    0.7 \\
    4716. & [NeIV]          &  0.040  & $<$    1.5 & $<$    1.6  &        -   &        -    & $<$    1.5 & $<$    1.6  & $<$    2.0 & $<$    2.0  & $<$    1.0 & $<$    1.0 \\
    4726. & [NeIV]          &  0.037  & $<$    1.5 & $<$    1.6  &        -   &        -    & $<$    1.5 & $<$    1.6  & $<$    2.0 & $<$    2.0  & $<$    1.0 & $<$    1.0 \\
    4741. & [ArIV]          &  0.033  &        2.7 &        2.9  &        -   &        -    &        3.9 &        4.1  & $<$    2.0 & $<$    2.0  & $<$    1.0 & $<$    1.0 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4959. & [OIII]          & -0.025  &      196.0 &      196.2  &      203.0 &      203.0  &       90.9 &       92.3  &      252.0 &      252.0  &      147.0 &      146.7 \\
    5007. & [OIII]          & -0.038  &      582.0 &      575.4  &      617.0 &      617.0  &      271.0 &      273.7  &      678.0 &      678.0  &      439.0 &      437.9 \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &       10.2 &        9.6  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        -   &        -    &        4.0 &        3.9  &        -   &        -    &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &        6.2 &        5.2  &        -   &        -    &        8.2 &        7.7  & $<$    0.5 & $<$    0.5  &        0.7 &        0.7 \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       12.5 &       10.2  &       15.6 &       15.6  &       18.7 &       17.4  &       13.2 &       13.2  &       11.5 &       11.3 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &       18.0 &       13.7  &        2.0 &        2.0  &        4.2 &        3.8  &        -   &        -    &       14.6 &       14.3 \\
    6312. & [SIII]+HeII     & -0.296  & $<$    3.0 & $<$    2.3  &        -   &        -    &        2.3 &        2.0  & $<$    1.0 & $<$    1.0  & $<$    0.3 & $<$    0.3 \\
    6365. & [OI]            & -0.304  &        4.7 &        3.5  &        -   &        -    &        -   &        -    &        -   &        -    &        4.3 &        4.2 \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  & $~$  106.0 & $~$   77.8  &        1.4 &        1.4  &       65.4 &       58.1  &        -   &        -    &       15.0 &       14.7 \\
    6563. & Halpha          & -0.334  &      396.0 &      282.3  &      282.0 &      282.0  &      315.0 &      272.2  &      279.0 &      279.0  &      270.0 &      263.8 \\
    6584. & [NII]           & -0.337  &      374.0 &      273.0  &        4.2 &        4.2  &      170.0 &      150.6  & $<$    1.0 & $<$    1.0  &       47.1 &       46.0 \\
    6678. & HeI+HeII        & -0.350  &        -   &        -    &        3.9 &        3.9  &        4.4 &        3.9  &        2.8 &        2.8  &        2.8 &        2.7 \\
    6716. & [SII]           & -0.356  &       13.1 &        9.4  &        -   &        -    &        2.8 &        2.5  & $<$    0.5 & $<$    0.5  &       12.1 &       11.8 \\
    6730. & [SII]           & -0.358  &       11.5 &        8.2  &        -   &        -    &        6.1 &        5.3  &        0.7 &        0.7  &       11.7 &       11.4 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$    5.0 & $<$    3.4  &        -   &        -    & $<$    2.0 & $<$    1.7  & $<$    0.5 & $<$    0.5  & $<$    0.3 & $<$    0.3 \\
    7065. & HeI             & -0.402  &        -   &        -    &        -   &        -    &       10.1 &        8.7  &        2.8 &        2.8  &        2.7 &        2.6 \\
    7136. & [ArIII]         & -0.410  &        7.6 &        5.1  &        -   &        -    &        7.0 &        6.0  &        1.0 &        1.0  &        2.8 &        2.8 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  & $<$    4.0 & $<$    2.7  &        -   &        -    &        1.6 &        1.3  & $<$    0.5 & $<$    0.5  &        4.1 &        3.9 \\
    7330. & [OII]           & -0.434  & $<$    4.0 & $<$    2.6  &        -   &        -    &        2.0 &        1.7  & $<$    0.5 & $<$    0.5  &        3.2 &        3.2 \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{     316. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{     759. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{     302. } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ 5.0 \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ 4.0 \%} & \multicolumn{2}{c}{ 8.0 \%} & \multicolumn{2}{c}{ 8.0 \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &        329.  & &          0.  & &      20678.  & &  $:$  1905.  & &        506.  & \\
%  &   Ne- [OII]   :    & &  $<$   727.  & &          0.  & &  $>$ 12779.  & &  $:$     0.  & &        862.  & \\
%  &   Ne- [ArIV]  :    & &       7969.  & &          0.  & &       7657.  & &  $:$     0.  & &  $:$     0.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{      300.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{    20700.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{      500.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    18000.} & \multicolumn{2}{c}{    13100.} & \multicolumn{2}{c}{    19200.} & \multicolumn{2}{c}{    14700.} & \multicolumn{2}{c}{    13000.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{    11000.} & \multicolumn{2}{c}{$:$ 13100.} & \multicolumn{2}{c}{    14600.} & \multicolumn{2}{c}{$:$ 14700.} & \multicolumn{2}{c}{    10000.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.44} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.19} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.03} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{MGPN\_SMC\_1  } & \multicolumn{2}{|c|}{MGPN\_SMC\_2  } & \multicolumn{2}{|c|}{MGPN\_SMC\_3  } & \multicolumn{2}{|c|}{MGPN\_SMC\_5  } & \multicolumn{2}{|c|}{MGPN\_SMC\_6  } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1550. & CIV             &  2.530  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1640. & HeII            &  2.319  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1663. & OIII]           &  2.267  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1750. & NIII]           &  2.071  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1909. & CIII]           &  1.793  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3727. & [OII]d          &  0.289  &      252.0 &      285.9  &       15.7 &       37.5  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   16.3  & $<$   40.0 & $<$   50.4 \\
    3798. & H10+HeII        &  0.271  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3869. & [NeIII]         &  0.253  & $<$   20.0 & $<$   22.3  &       20.7 &       44.4  &       26.5 &       26.5  & $<$   15.0 & $<$   16.2  & $<$   40.0 & $<$   49.4 \\
    3889. & H8+HeI+HeII     &  0.248  &        -   &        -    &        -   &        -    &       19.1 &       19.1  &        -   &        -    &        -   &        -   \\
    3969. & [NeIII]+H7      &  0.229  &        -   &        -    &       16.5 &       32.9  &       28.5 &       28.5  &       18.4 &       19.8  &        -   &        -   \\
    4026. & HeI+HeII        &  0.216  &        -   &        -    &        9.9 &       19.0  &        -   &        -    &        -   &        -    &        -   &        -   \\
    4070. & [SII]d          &  0.207  &        -   &        -    &        9.6 &       17.9  &        -   &        -    &       14.5 &       15.6  &        -   &        -   \\
    4102. & Hdelta          &  0.200  &       28.4 &       31.0  &        8.7 &       15.9  &       35.8 &       35.8  &       25.9 &       26.5  &        -   &        -   \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       56.4 &       60.3  &       21.6 &       34.1  &       66.9 &       66.9  &       51.0 &       51.9  &       40.2 &       44.0 \\
    4363. & [OIII]          &  0.147  &        -   &        -    &        -   &        -    & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   16.0  & $<$   40.0 & $<$   46.3 \\
    4471. & HeI             &  0.112  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4541. & HeII            &  0.091  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  & $<$   20.0 & $<$   20.4  & $<$    8.0 & $<$    9.2  & $<$   20.0 & $<$   20.0  &       95.5 &      100.9  &      114.0 &      124.4 \\
    4712. & [ArIV]          &  0.041  & $<$   20.0 & $<$   20.4  & $<$    8.0 & $<$    9.0  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.8  & $<$   40.0 & $<$   43.5 \\
    4716. & [NeIV]          &  0.040  & $<$   20.0 & $<$   20.3  & $<$    8.0 & $<$    9.0  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.8  & $<$   40.0 & $<$   43.4 \\
    4726. & [NeIV]          &  0.037  & $<$   20.0 & $<$   20.3  & $<$    8.0 & $<$    8.9  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.8  & $<$   40.0 & $<$   43.4 \\
    4741. & [ArIV]          &  0.033  & $<$   20.0 & $<$   20.3  & $<$    8.0 & $<$    8.8  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.8  & $<$   40.0 & $<$   43.3 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4959. & [OIII]          & -0.025  &      218.0 &      215.6  &      207.0 &      191.7  &      191.0 &      191.0  &      119.0 &      124.6  &      136.0 &      142.1 \\
    5007. & [OIII]          & -0.038  &      626.0 &      615.8  &      600.0 &      535.8  &      516.0 &      516.0  &      357.0 &      373.3  &      373.0 &      386.8 \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  & $<$   20.0 & $<$   18.1  & $<$    8.0 & $<$    4.1  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.4  & $<$   40.0 & $<$   37.1 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &       40.8 &       36.3 \\
    6312. & [SIII]+HeII     & -0.296  & $<$   20.0 & $<$   17.6  & $<$    8.0 & $<$    3.3  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.2  & $<$   40.0 & $<$   35.5 \\
    6365. & [OI]            & -0.304  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6563. & Halpha          & -0.334  &      329.0 &      284.3  &      564.0 &      206.0  &      269.0 &      269.0  &      295.0 &      283.9  &      325.0 &      266.1 \\
    6584. & [NII]           & -0.337  &       70.7 &       61.0  & $<$    8.0 & $<$    2.9  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.2  & $<$   40.0 & $<$   34.7 \\
    6678. & HeI+HeII        & -0.350  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6716. & [SII]           & -0.356  & $<$   20.0 & $<$   17.1  & $<$    8.0 & $<$    2.7  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.1  & $<$   40.0 & $<$   34.3 \\
    6730. & [SII]           & -0.358  & $<$   20.0 & $<$   17.1  & $<$    8.0 & $<$    2.7  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.1  & $<$   40.0 & $<$   34.3 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  & $<$   20.0 & $<$   16.8  & $<$    8.0 & $<$    2.4  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.1  & $<$   40.0 & $<$   33.5 \\
    7065. & HeI             & -0.402  &        -   &        -    &       32.4 &        9.6  &        -   &        -    &        -   &        -    &        -   &        -   \\
    7136. & [ArIII]         & -0.410  & $<$   20.0 & $<$   16.7  &       41.3 &       12.0  & $<$   20.0 & $<$   20.0  & $<$   15.0 & $<$   15.0  & $<$   40.0 & $<$   33.2 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7330. & [OII]           & -0.434  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & \\
%  &   Ne- [OII]   :    & &  $<$  1969.  & &  $<$  1955.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & \\
%  &   Ne- [ArIV]  :    & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.19} & \multicolumn{2}{c}{      1.31} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.05} & \multicolumn{2}{c}{      0.26} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{MGPN\_SMC\_7  } & \multicolumn{2}{|c|}{MGPN\_SMC\_8  } & \multicolumn{2}{|c|}{MGPN\_SMC\_9  } & \multicolumn{2}{|c|}{MGPN\_SMC\_10  } & \multicolumn{2}{|c|}{MGPN\_SMC\_11  } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1550. & CIV             &  2.530  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1640. & HeII            &  2.319  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1663. & OIII]           &  2.267  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1750. & NIII]           &  2.071  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1909. & CIII]           &  1.793  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3203. & HeII            &  0.498  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  &        -   &        -    &        -   &        -    & $<$    5.0 & $<$   13.4  &        -   &        -    &        -   &        -   \\
    3727. & [OII]d          &  0.289  &      297.0 &      569.8  &      425.0 &      425.0  &       11.6 &       23.8  & $<$   11.0 & $<$   12.6  &      322.0 &      322.0 \\
    3798. & H10+HeII        &  0.271  & $<$    1.0 & $<$    1.8  &        -   &        -    &        1.1 &        2.2  &        -   &        -    &        -   &        -   \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        8.2 &       14.8  &        -   &        -    &        2.1 &        4.0  &        -   &        -    &        -   &        -   \\
    3869. & [NeIII]         &  0.253  &       70.7 &      125.1  & $<$    5.0 & $<$    5.0  &       17.4 &       32.6  & $<$   11.0 & $<$   12.5  &       66.9 &       66.9 \\
    3889. & H8+HeI+HeII     &  0.248  &       20.9 &       36.6  &       21.4 &       21.4  &        9.0 &       16.7  &        -   &        -    &       29.3 &       29.3 \\
    3969. & [NeIII]+H7      &  0.229  &       36.9 &       61.9  &       13.1 &       13.1  &       14.0 &       24.8  &       23.3 &       26.2  &        -   &        -   \\
    4026. & HeI+HeII        &  0.216  &        2.1 &        3.4  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4070. & [SII]d          &  0.207  &        -   &        -    &        -   &        -    &        -   &        -    &       11.5 &       12.9  &        -   &        -   \\
    4102. & Hdelta          &  0.200  &       17.6 &       27.6  &       25.4 &       25.4  &       15.0 &       24.6  &       18.9 &       20.0  &       34.6 &       34.6 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       48.7 &       68.5  &       49.5 &       49.5  &       31.2 &       45.4  &       45.2 &       47.1  &       51.1 &       51.1 \\
    4363. & [OIII]          &  0.147  &        8.5 &       11.8  & $<$    5.0 & $<$    5.0  &       10.0 &       14.4  & $<$   11.0 & $<$   12.1  & $<$   30.0 & $<$   30.0 \\
    4471. & HeI             &  0.112  &        3.9 &        5.1  &        -   &        -    &        3.3 &        4.3  &        -   &        -    &        -   &        -   \\
    4541. & HeII            &  0.091  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        -   &        -    &        -   &        -    &        1.0 &        1.2  &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  &       17.6 &       19.6  &       28.5 &       28.5  & $<$    0.5 & $<$    0.6  &      106.0 &      113.4  & $<$   30.0 & $<$   30.0 \\
    4712. & [ArIV]          &  0.041  &        -   &        -    & $<$    5.0 & $<$    5.0  & $<$    0.5 & $<$    0.2  & $<$   11.0 & $<$   11.7  & $<$   30.0 & $<$   30.0 \\
    4716. & [NeIV]          &  0.040  &        -   &        -    & $<$    5.0 & $<$    5.0  & $<$    0.5 & $<$    0.6  & $<$   11.0 & $<$   11.7  & $<$   30.0 & $<$   30.0 \\
    4726. & [NeIV]          &  0.037  &        -   &        -    & $<$    5.0 & $<$    5.0  & $<$    0.5 & $<$    0.5  & $<$   11.0 & $<$   11.7  & $<$   30.0 & $<$   30.0 \\
    4741. & [ArIV]          &  0.033  & $<$    1.0 & $<$    1.1  & $<$    5.0 & $<$    5.0  & $<$    0.5 & $<$    0.5  & $<$   11.0 & $<$   11.7  & $<$   30.0 & $<$   30.0 \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        2.6 &        2.5  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4959. & [OIII]          & -0.025  &      190.0 &      179.4  &       35.4 &       35.4  &      143.0 &      134.2  &       77.8 &       81.6  &      260.0 &      260.0 \\
    5007. & [OIII]          & -0.038  &      646.0 &      593.5  &      100.0 &      100.0  &      442.0 &      402.6  &      244.0 &      255.0  &      744.0 &      744.0 \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &        -   &        -    &        -   &        -    & $~$    0.7 & $~$    0.4  &        -   &        -    &        -   &        -   \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       19.8 &       12.0  & $<$    5.0 & $<$    5.0  &       21.6 &       12.4  & $<$   11.0 & $<$   10.9  & $<$   30.0 & $<$   30.0 \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &       31.5 &       16.2  &        -   &        -    &        3.5 &        1.7  &        -   &        -    &        -   &        -   \\
    6312. & [SIII]+HeII     & -0.296  &        -   &        -    & $<$    5.0 & $<$    5.0  &        3.2 &        1.6  & $<$   11.0 & $<$   10.7  & $<$   30.0 & $<$   30.0 \\
    6365. & [OI]            & -0.304  &        6.3 &        3.2  &        -   &        -    &        2.0 &        1.0  &        -   &        -    &        -   &        -   \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  &       56.0 &       26.5  &       29.7 &       29.7  & $~$    6.0 & $~$    2.6  &        -   &        -    &       57.6 &       57.6 \\
    6563. & Halpha          & -0.334  &      592.0 &      278.7  &      257.0 &      257.0  &      605.0 &      263.7  &      252.0 &      229.8  &      285.0 &      285.0 \\
    6584. & [NII]           & -0.337  &      168.0 &       78.5  &      117.0 &      117.0  &        9.0 &        3.9  & $<$   11.0 & $<$   10.6  &      116.0 &      116.0 \\
    6678. & HeI+HeII        & -0.350  &        7.2 &        3.3  &        -   &        -    &        6.8 &        2.9  &        -   &        -    &        -   &        -   \\
    6716. & [SII]           & -0.356  &       27.5 &       12.3  &        5.9 &        5.9  &        2.2 &        0.9  & $<$   11.0 & $<$   10.5  & $<$   30.0 & $<$   30.0 \\
    6730. & [SII]           & -0.358  &       22.5 &       10.0  &       17.5 &       17.5  &        3.7 &        1.5  & $<$   11.0 & $<$   10.5  & $<$   30.0 & $<$   30.0 \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  &        9.9 &        4.1  & $<$    5.0 & $<$    5.0  & $<$    0.5 & $<$    0.2  & $<$   11.0 & $<$   10.4  & $<$   30.0 & $<$   30.0 \\
    7065. & HeI             & -0.402  &        4.2 &        1.7  &        -   &        -    &       22.3 &        8.2  &        -   &        -    &        -   &        -   \\
    7136. & [ArIII]         & -0.410  &        9.4 &        3.7  & $<$    5.0 & $<$    5.0  &       15.4 &        5.5  & $<$   11.0 & $<$   10.4  & $<$   30.0 & $<$   30.0 \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        2.5 &        0.9  &        -   &        -    &        2.1 &        0.7  &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  &        -   &        -    &        9.4 &        9.4  &       16.0 &        5.5  &        -   &        -    &        -   &        -   \\
    7330. & [OII]           & -0.434  &        6.4 &        2.4  &        6.9 &        6.9  &       12.4 &        4.2  &        -   &        -    &        -   &        -   \\
    7751. & [ArIII]         & -0.480  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        9.3 &        2.4  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &       10.8 &        2.6  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{     195. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{    1585. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{10.0 \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ 4.0 \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &        225.  & &     300000.  & &       4624.  & &  $:$     0.  & &  $:$     0.  & \\
%  &   Ne- [OII]   :    & &     *******  & &        779.  & &      16321.  & &  $:$     0.  & &  $<$  4374.  & \\
%  &   Ne- [ArIV]  :    & &  $<$     0.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & &  $:$     0.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{      200.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{     4600.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    15500.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{    20900.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{$:$ 15500.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$:$ 20900.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.98} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      1.08} & \multicolumn{2}{c}{      0.12} & \multicolumn{2}{c}{      0.00} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \addtocounter{table}{-1}
 \begin{table}
  \centering
  \scriptsize
  \caption{SMC PNe line intensities}
  \begin{tabular}{|c|l|c|rr|rr|rr|rr|rr|}
   \noalign{\bigskip}
   \hline\noalign{\smallskip}
\multicolumn{3}{|l|}{} & \multicolumn{2}{|c|}{MGPN\_SMC\_12  } & \multicolumn{2}{|c|}{MGPN\_SMC\_13  } & \multicolumn{2}{|c|}{[M95]\_1  } & \multicolumn{2}{|c|}{[M95]\_2  } & \multicolumn{2}{|c|}{LHA\_115-N\_8   } \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
 $\lambda$ & Lines & f($\lambda$) & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ & $I_{obs}$ & $I_{cor}$ \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
    1486. & NIV]            &  2.731  & $<$   50.0 & $<$ 1738.6  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1550. & CIV             &  2.530  & $<$   50.0 & $<$ 1341.1  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1640. & HeII            &  2.319  &       97.0 &     1980.7  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1663. & OIII]           &  2.267  & $<$   50.0 & $<$  954.8  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1750. & NIII]           &  2.071  & $<$   80.0 & $<$ 1187.8  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    1909. & CIII]           &  1.793  &      298.0 &     3089.7  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3203. & HeII            &  0.498  &        9.4 &       18.4  &       24.0 &       34.8  &        -   &        -    &        -   &        -    &        -   &        -   \\
    3347. & [NeV]           &  0.431  &        7.8 &       14.1  &        6.9 &        9.6  &        -   &        -    &        -   &        -    &        -   &        -   \\
    3427. & [NeV]           &  0.396  &       24.5 &       42.0  &       29.1 &       39.5  &        -   &        -    &        -   &        -    &        -   &        -   \\
    3727. & [OII]d          &  0.289  &       35.4 &       52.8  &        6.4 &        8.1  & $<$   24.0 & $<$   24.0  &      182.0 &      351.5  &      484.0 &      484.0 \\
    3798. & H10+HeII        &  0.271  &        -   &        -    &        2.4 &        3.0  &        -   &        -    &        -   &        -    &        -   &        -   \\
    3820. & HeI             &  0.265  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    3835. & H9+HeII         &  0.261  &        2.9 &        4.2  &        4.9 &        6.1  &        -   &        -    &        -   &        -    &        -   &        -   \\
    3869. & [NeIII]         &  0.253  &       49.2 &       70.0  &       16.5 &       20.4  &       59.6 &       59.6  &       58.3 &      103.8  &        -   &        -   \\
    3889. & H8+HeI+HeII     &  0.248  &       20.5 &       29.0  &        9.2 &       11.4  &       21.7 &       21.7  &        -   &        -    &        -   &        -   \\
    3969. & [NeIII]+H7      &  0.229  &       29.3 &       40.5  &       19.2 &       23.4  &       39.0 &       39.0  &       23.5 &       39.6  &        -   &        -   \\
    4026. & HeI+HeII        &  0.216  &        2.7 &        3.7  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4070. & [SII]d          &  0.207  &        4.5 &        6.0  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4102. & Hdelta          &  0.200  &       21.2 &       27.4  &       25.6 &       29.1  &       24.8 &       24.8  &       12.8 &       20.2  &       63.2 &       63.2 \\
    4199. & HeII            &  0.179  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4267. & CII             &  0.165  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4340. & Hgamma          &  0.151  &       42.2 &       51.3  &       43.3 &       47.7  &       69.3 &       69.3  &       33.4 &       47.1  &       52.8 &       52.8 \\
    4363. & [OIII]          &  0.147  &        8.7 &       10.7  &        7.5 &        8.7  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$   16.8  &        -   &        -   \\
    4471. & HeI             &  0.112  &        6.5 &        7.7  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4541. & HeII            &  0.091  &        2.9 &        3.4  &        4.1 &        4.6  &        -   &        -    &        -   &        -    &        -   &        -   \\
    4641. & NIII            &  0.061  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4649. & CIII            &  0.059  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4659. & CIV             &  0.056  &        2.8 &        3.1  &        5.2 &        5.6  &        -   &        -    &        -   &        -    &        -   &        -   \\
    4686. & HeII            &  0.048  &       52.8 &       57.7  &       97.5 &      105.7  & $<$   24.0 & $<$   24.0  &       40.3 &       45.0  &        -   &        -   \\
    4712. & [ArIV]          &  0.041  &        8.4 &        8.2  &        3.7 &        4.0  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$   13.2  &        -   &        -   \\
    4716. & [NeIV]          &  0.040  & $<$    1.5 & $<$    1.6  & $<$    1.0 & $<$    1.1  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$   13.1  &        -   &        -   \\
    4726. & [NeIV]          &  0.037  & $<$    1.5 & $<$    1.6  & $<$    1.0 & $<$    1.1  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$   13.0  &        -   &        -   \\
    4741. & [ArIV]          &  0.033  &        4.0 &        4.3  &        2.9 &        3.1  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$   12.9  &        -   &        -   \\
    4861. & Hbeta           &  0.000  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0  &      100.0 &      100.0 \\
    4922. & HeI             & -0.016  &        2.0 &        2.0  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    4959. & [OIII]          & -0.025  &       91.6 &       91.1  &       93.6 &       96.8  &      237.0 &      237.0  &      172.0 &      162.3  &        -   &        -   \\
    5007. & [OIII]          & -0.038  &      285.0 &      278.9  &      284.0 &      291.5  &      756.0 &      756.0  &      506.0 &      464.5  &        -   &        -   \\
    5193. & [ArIII]         & -0.082  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5200. & [NI]            & -0.084  &        8.3 &        7.7  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5412. & HeII            & -0.131  &        6.2 &        5.4  &        8.7 &        8.4  &        -   &        -    &        -   &        -    &        -   &        -   \\
    5519. & [ClIII]         & -0.154  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5539. & [ClIII]         & -0.158  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5578. & [OI]            & -0.166  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5755. & [NII]           & -0.200  &       14.4 &       11.4  & $<$    0.5 & $<$    0.5  &        -   &        -    &        -   &        -    &        -   &        -   \\
    5806. & CIV             & -0.210  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    5876. & HeI             & -0.222  &       26.4 &       20.4  &        1.1 &        1.0  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$    7.2  &        -   &        -   \\
    6088. & [CaV]+[FeVII]   & -0.260  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6103. & [KIV]           & -0.262  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6302. & [OI]            & -0.294  &        9.3 &        6.5  &        1.9 &        1.7  &        -   &        -    &        -   &        -    &        -   &        -   \\
    6312. & [SIII]+HeII     & -0.296  &        3.9 &        2.8  &        1.2 &        1.0  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$    6.1  &        -   &        -   \\
    6365. & [OI]            & -0.304  &        2.3 &        1.6  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6436. & [ArV]           & -0.315  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    6548. & [NII]           & -0.332  &      215.0 &      144.0  &        -   &        -    &        -   &        -    &       27.2 &       12.8  &       14.7 &       14.7 \\
    6563. & Halpha          & -0.334  &      454.0 &      295.2  &      344.0 &      277.4  &      234.0 &      234.0  &        -   &        -    &      282.0 &      282.0 \\
    6584. & [NII]           & -0.337  &      610.0 &      405.8  &        1.6 &        1.3  & $<$   24.0 & $<$   24.0  &      100.0 &       46.4  &       42.9 &       42.9 \\
    6678. & HeI+HeII        & -0.350  &        9.0 &        5.9  &        1.1 &        1.0  &        -   &        -    &        -   &        -    &        -   &        -   \\
    6716. & [SII]           & -0.356  &       23.6 &       15.3  & $<$    0.5 & $<$    0.4  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$    5.3  &       32.1 &       32.1 \\
    6730. & [SII]           & -0.358  &       29.4 &       19.0  & $~$    0.7 & $~$    0.6  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$    5.3  &        -   &        -   \\
    6897. & HeII            & -0.380  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7007. & [ArV]           & -0.394  &        1.8 &        1.1  &        1.4 &        1.1  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$    4.9  &        -   &        -   \\
    7065. & HeI             & -0.402  &       11.3 &        6.9  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7136. & [ArIII]         & -0.410  &       16.2 &        9.8  &        2.6 &        2.1  & $<$   24.0 & $<$   24.0  & $<$   12.0 & $<$    4.7  &        -   &        -   \\
    7172. & [ArIV]          & -0.415  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7281. & HeI             & -0.428  &        1.2 &        0.7  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    7320. & [OII]           & -0.433  &        -   &        -    & $<$    0.5 & $<$    0.4  &        -   &        -    &        -   &        -    &        -   &        -   \\
    7330. & [OII]           & -0.434  &        -   &        -    & $<$    0.5 & $<$    0.4  &        -   &        -    &        -   &        -    &        -   &        -   \\
    7751. & [ArIII]         & -0.480  &        5.1 &        2.8  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9069. & [SIII]          & -0.597  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
    9532. & [SIII]          & -0.631  &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -    &        -   &        -   \\
   \noalign{\smallskip}
   \hline\noalign{\smallskip}
   \noalign{\bigskip}
   \noalign{\bigskip}
\multicolumn{3}{l}{$H_{\beta}$ ($10^{-16}.erg.cm^{-2}.s^{-1}$)} & \multicolumn{2}{c}{     200. } & \multicolumn{2}{c}{     309. } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } & \multicolumn{2}{c}{ -        } \\
   \noalign{\smallskip}
\multicolumn{3}{l}{Uncertainty} & \multicolumn{2}{c}{ 4.0 \%} & \multicolumn{2}{c}{ 5.0 \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} & \multicolumn{2}{c}{ -   \%} \\
   \noalign{\smallskip}
   \noalign{\bigskip}
%  &   Ne- [SII]   :    & &       1350.  & &  $:$  2249.  & &  $:$     0.  & &  $:$     0.  & &          0.  & \\
%  &   Ne- [OII]   :    & &       3860.  & &  $<$  2276.  & &  $:$     0.  & &  $<$*******  & &          0.  & \\
%  &   Ne- [ArIV]  :    & &        100.  & &       1010.  & &  $:$     0.  & &  $:$     0.  & &          0.  & \\
%  &   Ne- [ClIII] :    & &          0.  & &          0.  & &          0.  & &          0.  & &          0.  & \\
\multicolumn{3}{l}{Ne-         : } & \multicolumn{2}{c}{     1300.} & \multicolumn{2}{c}{     1000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} & \multicolumn{2}{c}{$*$  5000.} \\
\multicolumn{3}{l}{Temp [OIII] : } & \multicolumn{2}{c}{    22100.} & \multicolumn{2}{c}{    18800.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} \\
\multicolumn{3}{l}{Temp [NII]  : } & \multicolumn{2}{c}{    12800.} & \multicolumn{2}{c}{$:$ 18800.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} & \multicolumn{2}{c}{$*$ 12000.} \\
\multicolumn{3}{l}{C opt       : } & \multicolumn{2}{c}{      0.56} & \multicolumn{2}{c}{      0.28} & \multicolumn{2}{c}{      0.00} & \multicolumn{2}{c}{      0.99} & \multicolumn{2}{c}{      0.00} \\
  \end{tabular}
  \normalsize
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newpage
 \clearpage
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

